Meta-Cognitive Analysis: Evaluating Declarative and Procedural Knowledge in Datasets and Large Language Models

Declarative knowledge and procedural knowledge are two key parts in meta-cognitive theory, and these two hold significant importance in pre-training and inference of LLMs. However, a comprehensive analysis comparing these two types of knowledge is lacking, primarily due to challenges in definition, probing and quantitative assessment. In this paper, we explore from a new perspective by providing ground-truth knowledge for LLMs and evaluating the effective score. Through extensive experiments with widely-used datasets and models, we get conclusions: (1) In most tasks, benefits from declarative knowledge are greater than those from procedural knowledge. (2) Profits of procedural knowledge are larger than declarative knowledge only in reasoning tasks with simple logic. (3) As pre-training progresses and size increases, model ability to utilize both kinds of knowledge significantly improves, but in different speed. We do detailed analysis for the findings and this can provide primary guidance for evaluation and enhancement of large language models.

==> tables/model_input_examples.tex <==
\begin{table}[htbp]
\begin{center}
% \resizebox{1.0\linewidth}{!}{
\begin{tabularx}{\columnwidth}{|X|}
\hline
Generate reasoning for question based on procedural augment.\\
\\
(example1)\\
\textbf{Question:}\\
Jared is trying to increase his ...\\
\textbf{Procedural augment:}\\
Add the initial and increased typing ...\\
Predict the next typing speed by ...\\
Consider this prediction as another ...\\
To find the average, divide the total ...\\
\textbf{Reasoning:}\\
Add the initial ... Therefore, the answer is 52.\\
\\
(example2)\\
......\\
\\
\textbf{Question:}\\
data["question"]\\
\textbf{Procedural augment:}\\
data["procedural-augment"]\\
\textbf{Reasoning:}\\
\hline
% Generate reasoning for question. Some facts may be useful.\\
% \\
% Question:\\
% {examples[0]["question"]}\\
% Some facts:\\
% {hint0}\\
% Reasoning:\\
% {examples[0]["reasoning"]}\\

% Question:\\
% {examples[1]["question"]}\\
% Some facts:\\
% {hint1}\\
% Reasoning:\\
% {examples[1]["reasoning"]}\\
% \\
% Question:\\
% {data["question"]}\\
% Some facts:\\
% {hint}\\
% Reasoning:\\
% \hline
\end{tabularx}%}
\caption{One model input example for procedural knowledge. All the models and datasets use the same prompt format.}
\label{table:model-input-examples}
\end{center}
\end{table}

==> tables/p_part_f_part_examples.tex <==
\begin{table}[htbp]
\begin{center}
% \resizebox{1.0\linewidth}{!}{
\begin{tabularx}{\columnwidth}{|X|}
\hline
\textbf{Question:} \\ % 这种东西到底是用table还是figure？
Jared is trying to increase his typing speed. He starts with 47 words per minute (WPM). After some lessons the next time he tests his typing speed it has increased to 52 WPM. If he continues to increase his typing speed once more by 5 words, what will be the average of the three measurements?\\ \\
% \textbf{Answer:} \\
% 52\\ \\
\textbf{Procedural knowledge:}\\ 
Add the initial and increased typing speeds together to find a total.\\
Predict the next typing speed by adding 5 words per minute to the most recent speed.\\
Consider this prediction as another measurement and add it to the total.\\
To find the average, divide the total of the three measurements by the number of measurements.\\ \\
\textbf{Declarative knowledge:} \\
47 + 52 = 99 \\
52 + 5 = 57 \\
99 + 57 = 156 \\
156 / 3 = 52 \\
\hline
\end{tabularx}%}
\caption{One example about procedural knowledge and declarative knowledge from GSM8K.}
\label{table:p_part_f_part_examples}
\end{center}
\end{table}

